Blind Identification of Channel Codes: A Subspace-Coding Approach

The problem of blind identification of channel codes at a receiver involves identifying a code chosen by a transmitter from a known code-family, by observing the transmitted codewords through the channel. Most existing approaches for code-identification are contingent upon the codes in the family having some special structure, and are often computationally expensive otherwise. Further, rigorous analytical guarantees on the performance of these existing techniques are largely absent. This work presents a new method for code-identification on the binary symmetric channel (BSC), inspired by the framework of subspace codes for operator channels, carefully combining principles of hamming-metric and subspace-metric decoding. We refer to this method as the minimum denoised subspace discrepancy decoder. We present theoretical guarantees for code-identification using this decoder, for bounded-weight errors, and also present a bound on the probability of error when used on the BSC. Simulations demonstrate the improved performance of our decoder for random linear codes beyond existing general-purpose techniques, across most channel conditions and even with a limited number of received vectors.

==> Macros_CodeID_subspace.tex <==
\newcommand{\rowspaceof}{\mathsf{rowsp}}  % rowspaceofmatrix
\newcommand{\colspaceof}{\mathsf{colsp}}  % columnspaceofmatrix


\newcommand{\Fb}{\mathbb{F}} % field
\newcommand{\Zb}{\mathbb{Z}} % integers

\newcommand{\rank}{\mathsf{rank}} 

% \newcommand{\spanof}[1]{\langle #1 \rangle} 
\newcommand{\pk}[1]
{{\color{red} pk: #1}} % integers
\newcommand{\ps}[1]{{\color{magenta} Pramod: #1}}
% \newcommand{\ps}[1]{%
%   \iftoggle{showcomment}{%
%     {\color{magenta}[\fontfamily{cmss}\selectfont Pramod: #1]}%
%   }{}% 
% }
\newcommand{\Ber}{\mathsf{Ber}}


% Set of indices of non zero rows of a matrix
% \newcommand{\NI}{\mathcal{S}}
\newcommand{\NI}[1]{\mathbb{S}_{#1}}
%%%

\newcommand{\tth}{\mathsf{th}} %%superscript th

%------ submatrix formed by set of w rows of a matrix A 
\newcommand{\SM}[2]{#1_{#2}}
% k_th row of a matrix. 
\newcommand{\row}[2]{#1[{#2},:]} 

% k_th column of a matrix.
\newcommand{\col}[2]{#1[:,{#2}]}

% hamming weight of a vector 
\newcommand{\w}{\text{wt}_H}

%--- Span of a Matrix -----% 
\newcommand{\s}[1]{\left\langle #1 \right\rangle}

% Submatrix formed by selecting rows
% \newcommand{\rowsub}[2]{#1\!\left[#2\right]}
\newcommand{\MDens}{\mathsf{M-DenSD}}


